Observation of implicit complexity by non confluence

We propose to consider non confluence with respect to implicit complexity. We come back to some well known classes of first-order functional program, for which we have a characterization of their intentional properties, namely the class of cons-free programs, the class of programs with an interpretation, and the class of programs with a quasi-interpretation together with a termination proof by the product path ordering. They all correspond to PTIME. We prove that adding non confluence to the rules leads to respectively PTIME, NPTIME and PSPACE. Our thesis is that the separation of the classes is actually a witness of the intentional properties of the initial classes of programs.

==> eptcsdata.tex <==
\providecommand{\event}{P. Baillot (Ed.): Workshop on Developments in\\
 Implicit Computational complExity (DICE 2010). }
\providecommand{\volume}{23}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{15}
\providecommand{\eid}{2}

